The Effect of Tail Stiffness on a Sprawling Quadruped Locomotion

A distinctive feature of quadrupeds that is integral to their locomotion is the tail. Tails serve many purposes in biological systems including propulsion, counterbalance, and stabilization while walking, running, climbing, or jumping. Similarly, tails in legged robots may augment the stability and maneuverability of legged robots by providing an additional point of contact with the ground. However, in the field of terrestrial bio-inspired legged robotics, the tail is often ignored because of the difficulties in design and control. This study will test the hypothesis that a variable stiffness robotic tail can improve the performance of a sprawling quadruped robot by enhancing its stability and maneuverability in various environments. To test our hypothesis, we add a multi-segment, cable-driven, flexible tail, whose stiffness is controlled by a single servo motor in conjunction with a reel and cable system, to the underactuated sprawling quadruped robot. By controlling the stiffness of the tail, we have shown that the stability of locomotion on rough terrain and the climbing ability of the robot are improved compared to the movement with a rigid tail and no tail. The flexible tail design also provides passively controlled tail undulation capabilities through the robot's lateral movement, which contributes to stability.

==> bibtex.tex <==
\begin{thebibliography}{10}

\bibitem{arnold1984evolutionary}
Edwin~Nicholas Arnold.
\newblock Evolutionary aspects of tail shedding in lizards and their relatives.
\newblock {\em Journal of Natural History}, 18(1):127--169, 1984.

\bibitem{b2013impact}
Gary B.~Gillis, Chi-Yun Kuo, and Duncan Irschick.
\newblock The impact of tail loss on stability during jumping in green anoles
  (anolis carolinensis).
\newblock {\em Physiological and Biochemical Zoology}, 86(6):680--689, 2013.

\bibitem{TailQuadruped2021}
Pinhas Ben-Tzvi and Yujiong Liu.
\newblock {Robots with Tails}.
\newblock {\em Mechanical Engineering}, 143(6):32--37, 11 2021.

\bibitem{CheetahRobotStabilityTail}
Randall Briggs, Jongwoo Lee, Matt Haberland, and Sangbae Kim.
\newblock Tails in biomimetic design: Analysis, simulation, and experiment.
\newblock In {\em 2012 IEEE/RSJ International Conference on Intelligent Robots
  and Systems}, pages 1473--1480, 2012.

\bibitem{Brill2015}
Anna~L. Brill, Avik De, Aaron~M. Johnson, and Daniel~E. Koditschek.
\newblock Tail-assisted rigid and compliant legged leaping.
\newblock In {\em 2015 IEEE/RSJ International Conference on Intelligent Robots
  and Systems (IROS)}, pages 6304--6311, 2015.

\bibitem{QuadrupedRobotTurning}
Carlos Casarez, Ivan Penskiy, and Sarah Bergbreiter.
\newblock Using an inertial tail for rapid turns on a miniature legged robot.
\newblock In {\em 2013 IEEE International Conference on Robotics and
  Automation}, pages 5469--5474, 2013.

\bibitem{Casarez2017}
Carlos~S. Casarez and Ronald~S. Fearing.
\newblock Dynamic terrestrial self-righting with a minimal tail.
\newblock In {\em 2017 IEEE/RSJ International Conference on Intelligent Robots
  and Systems (IROS)}, pages 314--321, 2017.

\bibitem{chang2011lizard}
Evan Chang-Siu, Thomas Libby, Masayoshi Tomizuka, and Robert~J Full.
\newblock A lizard-inspired active tail enables rapid maneuvers and dynamic
  stabilization in a terrestrial robot.
\newblock In {\em 2011 IEEE/RSJ International Conference on Intelligent Robots
  and Systems}, pages 1887--1894. IEEE, 2011.

\bibitem{feilich2015passive}
Kara~L Feilich and George~V Lauder.
\newblock Passive mechanical models of fish caudal fins: effects of shape and
  stiffness on self-propulsion.
\newblock {\em Bioinspiration \& biomimetics}, 10(3):036002, 2015.

\bibitem{flammang2011volumetric}
Brooke~E Flammang, George~V Lauder, Daniel~R Troolin, and Tyson Strand.
\newblock Volumetric imaging of shark tail hydrodynamics reveals a
  three-dimensional dual-ring vortex wake structure.
\newblock {\em Proceedings of the Royal Society B: Biological Sciences},
  278(1725):3670--3678, 2011.

\bibitem{CapachinTail}
P.A. Garber and J.A. Rehg.
\newblock The ecological role of the prehensile tail in white-faced capuchins
  (cebus capucinus).
\newblock {\em American Journal of Physical Anthropology}, 110(3):325--339,
  1999.

\bibitem{garber1999ecological}
Paul~A Garber and Jennifer~A Rehg.
\newblock The ecological role of the prehensile tail in white-faced capuchins
  (cebus capucinus).
\newblock {\em American Journal of Physical Anthropology: The Official
  Publication of the American Association of Physical Anthropologists},
  110(3):325--339, 1999.

\bibitem{gillis2016consequences}
Gary Gillis and Timothy~E Higham.
\newblock Consequences of lost endings: caudal autotomy as a lens for focusing
  attention on tail function during locomotion.
\newblock {\em Journal of Experimental Biology}, 219(16):2416--2422, 2016.

\bibitem{RISEV3}
G.~Clark Haynes, Alex Khripin, Goran Lynch, Jonathan Amory, Aaron Saunders,
  Alfred~A. Rizzi, and Daniel~E. Koditschek.
\newblock Rapid pole climbing with a quadrupedal robot.
\newblock In {\em 2009 IEEE International Conference on Robotics and
  Automation}, pages 2767--2772, 2009.

\bibitem{MammalTailReview}
Graham~C. Hickman.
\newblock The mammalian tail: a review of functions.
\newblock {\em Mammal Review}, 9(4):143--157, 1979.

\bibitem{higham2013integrative}
Timothy~E Higham, Anthony~P Russell, and Peter~A Zani.
\newblock Integrative biology of tail autotomy in lizards.
\newblock {\em Physiological and Biochemical Zoology}, 86(6):603--610, 2013.

\bibitem{howell1944speed}
Alfred~Brazier Howell et~al.
\newblock Speed in animals, their specialization for running and leaping.
\newblock {\em Speed in animals, their specialization for running and
  leaping.}, 1944.

\bibitem{ibrahim2020tail}
Nizar Ibrahim, Simone Maganuco, Cristiano Dal~Sasso, Matteo Fabbri, Marco
  Auditore, Gabriele Bindellini, David~M Martill, Samir Zouhri, Diego~A
  Mattarelli, David~M Unwin, et~al.
\newblock Tail-propelled aquatic locomotion in a theropod dinosaur.
\newblock {\em Nature}, 581(7806):67--70, 2020.

\bibitem{johnson2012tail}
Aaron~M Johnson, Thomas Libby, Evan Chang-Siu, Masayoshi Tomizuka, Robert~J
  Full, and Daniel~E Koditschek.
\newblock Tail assisted dynamic self righting.
\newblock In {\em CLAWAR 2012 – Proceedings of the Fifteenth International
  Conference on Climbing and Walking Robots and the Support Technologies for
  Mobile Machines,}. 2012.

\bibitem{jusufi2010righting}
Ardian Jusufi, Daniel~T Kawano, Thomas Libby, and Robert~J Full.
\newblock Righting and turning in mid-air using appendage inertia: reptile
  tails, analytical models and bio-inspired robots.
\newblock {\em Bioinspiration \& biomimetics}, 5(4):045001, 2010.

\bibitem{karakasiliotis2009analysis}
Konstantinos Karakasiliotis and Auke~Jan Ijspeert.
\newblock Analysis of the terrestrial locomotion of a salamander robot.
\newblock In {\em 2009 IEEE/RSJ International Conference on Intelligent Robots
  and Systems}, pages 5015--5020. IEEE, 2009.

\bibitem{keenleyside2012diversity}
Miles~HA Keenleyside.
\newblock {\em Diversity and adaptation in fish behaviour}, volume~11.
\newblock Springer Science \& Business Media, 2012.

\bibitem{lauder2005hydrodynamics}
George~V Lauder and Eric~D Tytell.
\newblock Hydrodynamics of undulatory propulsion.
\newblock {\em Fish physiology}, 23:425--468, 2005.

\bibitem{libby2012tail}
Thomas Libby, Talia~Y Moore, Evan Chang-Siu, Deborah Li, Daniel~J Cohen, Ardian
  Jusufi, and Robert~J Full.
\newblock Tail-assisted pitch control in lizards, robots and dinosaurs.
\newblock {\em Nature}, 481(7380):181--184, 2012.

\bibitem{lighthill1969hydromechanics}
MJ~Lighthill.
\newblock Hydromechanics of aquatic animal propulsion.
\newblock {\em Annual review of fluid mechanics}, 1(1):413--446, 1969.

\bibitem{liu2021dynamic}
Yujiong Liu and Pinhas Ben-Tzvi.
\newblock Dynamic modeling, analysis, and comparative study of a quadruped with
  bio-inspired robotic tails.
\newblock {\em Multibody System Dynamics}, 51(2):195--219, 2021.

\bibitem{Lynch2012}
Goran~A Lynch, Jonathan~E Clark, Pei-Chun Lin, and Daniel~E Koditschek.
\newblock A bioinspired dynamical vertical climbing robot.
\newblock {\em The International Journal of Robotics Research}, 31(8):974--996,
  2012.

\bibitem{muddybot2016}
Benjamin McInroe, Henry~C. Astley, Chaohui Gong, Sandy~M. Kawano, Perrin~E.
  Schiebel, Jennifer~M. Rieser, Howie Choset, Richard~W. Blob, and Daniel~I.
  Goldman.
\newblock Tail use improves performance on soft substrates in models of early
  vertebrate land locomotors.
\newblock {\em Science}, 353(6295):154--158, 2016.

\bibitem{nabeshima2019prosthetic}
Junichi Nabeshima, MHD~Yamen Saraiji, and Kouta Minamizawa.
\newblock Prosthetic tail: Artificial anthropomorphic tail for extending innate
  body functions.
\newblock In {\em Proceedings of the 10th Augmented Human International
  Conference 2019}, pages 1--4, 2019.

\bibitem{naya2007some}
Daniel~E Naya, Claudio Veloso, Jos{\'e}~LP Mu{\~n}oz, and Francisco Bozinovic.
\newblock Some vaguely explored (but not trivial) costs of tail autotomy in
  lizards.
\newblock {\em Comparative Biochemistry and Physiology Part A: Molecular \&
  Integrative Physiology}, 146(2):189--193, 2007.

\bibitem{Norby2021}
Joseph Norby, Jun~Yang Li, Cameron Selby, Amir Patel, and Aaron~M. Johnson.
\newblock Enabling dynamic behaviors with aerodynamic drag in lightweight
  tails.
\newblock {\em IEEE Transactions on Robotics}, 37(4):1144--1153, 2021.

\bibitem{kangaroo2014}
Shawn~M. O'Connor, Terence~J. Dawson, Rodger Kram, and J.~Maxwell Donelan.
\newblock The kangaroo's tail propels and powers pentapedal locomotion.
\newblock {\em Biology Letters}, 10(7):20140381, 2014.

\bibitem{OzkanAydin2020Centipede}
Yasemin Ozkan-Aydin, Baxi Chong, Enes Aydin, and Daniel~I Goldman.
\newblock A systematic approach to creating terrain-capable hybrid soft/hard
  myriapod robots.
\newblock In {\em RoboSoft}, pages 156--163, 2020.

\bibitem{OzkanAydin_Swarm2021}
Yasemin Ozkan-Aydin and Daniel~I. Goldman.
\newblock Self-reconfigurable multilegged robot swarms collectively accomplish
  challenging terradynamic tasks.
\newblock {\em Science Robotics}, 6(56):eabf1628, 2021.

\bibitem{CheetahTailTurning}
Amir Patel and M.~Braae.
\newblock Rapid turning at high-speed: Inspirations from the cheetah's tail.
\newblock In {\em 2013 IEEE/RSJ International Conference on Intelligent Robots
  and Systems}, pages 5506--5511, 2013.

\bibitem{santori2005locomotion}
Ricardo~Tadeu Santori, Oscar Rocha-Barbosa, Marcus~Vin{\'\i}cius Vieira,
  Jos{\'e}~Aar{\~a}o Magnan-Neto, and Mariana~FC Loguercio.
\newblock Locomotion in aquatic, terrestrial, and arboreal habitat of
  thick-tailed opossum, lutreolina crassicaudata (desmarest, 1804).
\newblock {\em Journal of Mammalogy}, 86(5):902--908, 2005.

\bibitem{PrehensileTail}
Daniel Schmitt, Michael~D. Rose, Jean~E. Turnquist, and Pierre Lemelin.
\newblock Role of the prehensile tail during ateline locomotion: Experimental
  and osteological evidence.
\newblock {\em American Journal of Physical Anthropology}, 126(4):435--446,
  2005.

\bibitem{Schwaner2021}
M~J Schwaner, S~T Hsieh, I~Braasch, S~Bradley, C~B Campos, C~E Collins, C~M
  Donatelli, F~E Fish, O~E Fitch, B~E Flammang, B~E Jackson, A~Jusufi, P~J
  Mekdara, A~Patel, B~J Swalla, M~Vickaryous, and C~P McGowan.
\newblock {Future Tail Tales: A Forward-Looking, Integrative Perspective on
  Tail Research}.
\newblock {\em Integrative and Comparative Biology}, 61(2):521--537, 05 2021.

\bibitem{siddall2021mechanisms}
Robert Siddall, Victor Ibanez, Greg Byrnes, Robert~J Full, and Ardian Jusufi.
\newblock Mechanisms for mid-air reorientation using tail rotation in gliding
  geckos.
\newblock {\em Integrative and comparative biology}, 61(2):478--490, 2021.

\bibitem{TailTapRobot}
Daniel Soto, Kelimar Diaz, and Daniel~I. Goldman.
\newblock Enhancing legged robot navigation of rough terrain via tail tapping.
\newblock In Daisuke Chugo, Mohammad~Osman Tokhi, Manuel~F. Silva, Taro
  Nakamura, and Khaled Goher, editors, {\em Robotics for Sustainable Future},
  pages 213--225, Cham, 2022. Springer International Publishing.

\bibitem{walker1998balance}
Curt Walker, Charles~J Vierck~Jr, and Louis~A Ritz.
\newblock Balance in the cat: role of the tail and effects of sacrocaudal
  transection.
\newblock {\em Behavioural brain research}, 91(1-2):41--47, 1998.

\bibitem{willey2004tail}
Jeffrey~S Willey and Richard~W Blob.
\newblock Tail kinematics of juvenile common snapping turtles during aquatic
  walking.
\newblock {\em Journal of Herpetology}, 38(3):360--369, 2004.

\bibitem{TailStability}
Jesse~W Young, Brad~A Chadwell, Noah~T Dunham, Allison McNamara, Taylor Phelps,
  Tobin Hieronymus, and Liza~J Shapiro.
\newblock {The Stabilizing Function of the Tail During Arboreal
  Quadrupedalism}.
\newblock {\em Integrative and Comparative Biology}, 61(2):491--505, 06 2021.

\bibitem{young2015tail}
Jesse~W Young, Gabrielle~A Russo, Connie~D Fellmann, Meena~A Thatikunta, and
  Brad~A Chadwell.
\newblock Tail function during arboreal quadrupedalism in squirrel monkeys
  (saimiri boliviensis) and tamarins (saguinus oedipus).
\newblock {\em Journal of Experimental Zoology Part A: Ecological Genetics and
  Physiology}, 323(8):556--566, 2015.

\end{thebibliography}

